Return probability of quantum and correlated random walks

The analysis of the return probability is one of the most essential and fundamental topics in the study of classical random walks. In this paper, we study the return probability of quantum and correlated random walks in the one-dimensional integer lattice by the path counting method. We show that the return probability of both quantum and correlated random walks can be expressed in terms of the Legendre polynomial. Moreover, the generating function of the return probability can be written in terms of elliptic integrals of the first and second kinds for the quantum walk.

==> summary.tex <==
\section{Summary}
This paper is a continuation of our previous study \cite{Kiumi2021-yg}, which concentrates on the eigenvalues of the time evolution operator for two-phase QWs with one defect. 
In this paper, we focused on the quantitative study of localization and strong trapping property by deriving time-averaged limit distributions on space-inhomogeneous QWs on the integer lattice $\mathbb{Z}$. In Section \ref{sec:2}, we introduced the definitions of our model and gave the method to formulate eigenvectors of time evolution operator. Moreover, we showed some results to characterize eigenvalues not only for two-phase QWs with one defect but also for the more general space-inhomogeneous model. The necessary and sufficient condition for the eigenvectors was shown in Theorem \ref{Theorem Ker}. We also defined the strong trapping with the time-averaged limit distribution, which can be calculated with eigenvectors. In Section \ref{sec:3}, we derived eigenvectors and time-averaged limit distributions for five models whose eigenvalues were derived in the main theorems in the authors' previous study \cite{Kiumi2021-yg}. Models 1 and 2 are one-defect QWs, models 3 and 4 are two-phase QWs, and model 5 are two-phase QWs with one defect. Furthermore, the class of strong trapping was also revealed for these models. 
